Provably Efficient Primal-Dual Reinforcement Learning for CMDPs with Non-stationary Objectives and Constraints

We consider primal-dual-based reinforcement learning (RL) in episodic constrained Markov decision processes (CMDPs) with non-stationary objectives and constraints, which plays a central role in ensuring the safety of RL in time-varying environments. In this problem, the reward/utility functions and the state transition functions are both allowed to vary arbitrarily over time as long as their cumulative variations do not exceed certain known variation budgets. Designing safe RL algorithms in time-varying environments is particularly challenging because of the need to integrate the constraint violation reduction, safe exploration, and adaptation to the non-stationarity. To this end, we identify two alternative conditions on the time-varying constraints under which we can guarantee the safety in the long run. We also propose the \underline{P}eriodically \underline{R}estarted \underline{O}ptimistic \underline{P}rimal-\underline{D}ual \underline{P}roximal \underline{P}olicy \underline{O}ptimization (PROPD-PPO) algorithm that can coordinate with both two conditions. Furthermore, a dynamic regret bound and a constraint violation bound are established for the proposed algorithm in both the linear kernel CMDP function approximation setting and the tabular CMDP setting under two alternative conditions. This paper provides the first provably efficient algorithm for non-stationary CMDPs with safe exploration.

==> files/Experiments.tex <==
\section{Experiments}\label{sec:Experiments}

\subsection{Figures}

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{icml_numpapers}}
\caption{Historical locations and number of accepted papers for International
Machine Learning Conferences (ICML 1993 -- ICML 2008) and International
Workshops on Machine Learning (ML 1988 -- ML 1992). At the time this figure was
produced, the number of accepted papers for ICML 2008 was unknown and instead
estimated.}
\label{icml-historical}
\end{center}
\vskip -0.2in
\end{figure}

You may want to include figures in the paper to illustrate
your approach and results. Such artwork should be centered,
legible, and separated from the text. Lines should be dark and at
least 0.5~points thick for purposes of reproduction, and text should
not appear on a gray background.

Label all distinct components of each figure. If the figure takes the
form of a graph, then give a name for each axis and include a legend
that briefly describes each curve. Do not include a title inside the
figure; instead, the caption should serve this function.

Number figures sequentially, placing the figure number and caption
\emph{after} the graphics, with at least 0.1~inches of space before
the caption and 0.1~inches after it, as in
Figure~\ref{icml-historical}. The figure caption should be set in
9~point type and centered unless it runs two or more lines, in which
case it should be flush left. You may float figures to the top or
bottom of a column, and you may set wide figures across both columns
(use the environment \texttt{figure*} in \LaTeX). Always place
two-column figures at the top or bottom of the page.

\subsection{Tables}

You may also want to include tables that summarize material. Like
figures, these should be centered, legible, and numbered consecutively.
However, place the title \emph{above} the table with at least
0.1~inches of space before the title and the same after it, as in
Table~\ref{sample-table}. The table title should be set in 9~point
type and centered unless it runs two or more lines, in which case it
should be flush left.

% Note use of \abovespace and \belowspace to get reasonable spacing
% above and below tabular lines.

\begin{table}[t]
\caption{Classification accuracies for naive Bayes and flexible
Bayes on various data sets.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

Tables contain textual material, whereas figures contain graphical material.
Specify the contents of each row and column in the table's topmost
row. Again, you may float tables to a column's top or bottom, and set
wide tables across both columns. Place two-column tables at the
top or bottom of the page.


==> files/Proof_outline.tex <==
\section{Convergence analysis} \label{sec:proof outline}
In this section, we outline some of the key ideas behind the proof of Theorem \ref{thm: Linear Kernal MDP}, especially how to decouple the dynamic regret and constraint violation under the non-stationarity. We defer the
full proof of Theorems \ref{thm: Linear Kernal MDP} and \ref{thm: Tabular Case MDP} to Appendixes \ref{sec:appe-linear MDP} and \ref{sec:appe-tabular}, respectively.

\subsection{Dynamic regret analysis}
Our analysis for the dynamic regret begins with the decomposition of the regret given in \eqref{eq: d regret}:
\begin{align} \label{eq: decomposed d regret main paper} 
 &\text{D-Regret}(M)=\text{(R.\rom{1})}+\text{(R.\rom{2})}
\end{align}
where $\text{(R.\rom{1})}=\sum_{m=1}^M\left(V_{r,1}^{{\pi}^{\star,m},m}(x_1)-V_{r,1}^{m}(x_1) \right)$ and $\text{(R.\rom{2})}=\sum_{m=1}^M\left(V_{r,1}^{m}(x_1) -V_{r,1}^{\pi^m,m}(x_1)\right)$.

Note that with the policy-based method in \eqref{eq: PPO step}, the value estimation $V_{r,1}^{m}(x_1)$ is not necessarily an optimistic upper bound on the true optimal value function $V_{r,1}^{{\pi}^{\star,m},m}(x_1)$ as in the Q-learning based method. Thus, to analyze the first term $\text{(R.\rom{1})}$, we first define the model prediction error for the reward at episode $m$ as 
\begin{align*} 
   \iota_{\diamond, h}^{m} \coloneqq \diamond_h^m+ \mathbb{P}_h^m V_{\diamond,h+1}^m - Q_{\diamond,h}^m, \text{ for } \diamond = r \text{ or } g,
\end{align*}
for all $(m,h) \in [M] \times [H]$, which describes the error in the Bellman equation \eqref{eq: belmman equation} using $V_{\diamond,h+1}^m$ instead of $V_{\diamond,h+1}^{\pi^m,m}$ and using the sample estimation of $ \mathbb{P}_h^m$. Then, with the help of the performance difference lemma (Lemma \ref{lemma: expansion of V star m -V m}), the one-step descent lemma (Lemma \ref{lemma: One-step descent lemma}) and the appropriate choices of parameters, the policy update step  in Algorithm \ref{alg:algoirthm 1} yields the following improvement guarantee:
\begin{align} 
\nonumber&\text{(R.\rom{1})} \leq  \widetilde{\mathcal{O}} \left( H^3 M^{\frac{2}{3}} (\sqrt{d}B_\Delta+B_\star)^{\frac{1}{3}} \right) \\
 & - \sum_{m=1}^{M} \mu^{m}\left(V_{g, 1}^{\pi^{\star,m},m}\left(x_{1}\right)-V_{g, 1}^{m}\left(x_{1}\right)\right)  \label{eq: primal step main paper 1}+\\
&\sum_{m=1}^M\sum_{h=1}^H \EE_{{\pi}^{\star,m}, \mathbb{P}^m} \left[ \iota_{r, h}^{m}(x_h,a_h) +\mu^m \iota_{g, h}^{m}(x_h,a_h)\right].  \label{eq: primal step main paper 2}
\end{align}

The above inequality displays a decoupling between the regret (R.\rom{1}) and the constraint. This decoupling can also be found in \cite{ding2021provably,ding2020natural,mahdavi2012trading,wei2020online}. Then, we analyze the last two terms in  \eqref{eq: primal step main paper 2}  separately. Via the dual update in Algorithm \ref{alg:algoirthm 1}, one can verify that
\begin{align*}
-\sum_{m=1}^M \mu^m \left(V_{g, 1}^{{\pi}^{*,m}, m}\left(x_{1}\right)-V_{g, 1}^{m}\left(x_{1}\right)\right) \leq   \mathcal{O}\left(H^2M^{\frac{1}{2}}\right).  
\end{align*}


% Since both the running policy $\Tilde{\pi}^m$ and the benchmark  $\Tilde{\pi}^{\star,m}$ are in the interior of the simplex $\Delta(\mathcal{A} \mid \mathcal{S}, H)$, we can guarantee the boundedness of the telescoping of the drifting KL divergence.
% \begin{lemma}
% Let assumptions of Theorem ?? hold. Then, 
% $\frac{1}{\alpha}\sum_{m=1}^M  \sum_{h=1}^{H} \mathbb{E}_{\Tilde{\pi}^{\star,m}, \mathbb{P}^{m}}\left[D\left(\Tilde{\pi}_h^{\star,m} \mid \tilde{\pi}_{h}^{m}\right)-D\left(\Tilde{\pi}_h^{\star,m} \mid \tilde{\pi}_{h}^{m+1}\right)\right]
%   \leq $
% \end{lemma}
% The above lemma also implies the importance of using an exploratory policy in the non-stationary environment. 
The last term of \eqref{eq: primal step main paper 2} is due to the model prediction error and can be bounded together with the term (R.\rom{2}) in \eqref{eq: decomposed d regret} which can be expanded into 
\begin{align*} 
\text{(R.\rom{2})}=-\sum_{m=1}^{M} \sum_{h=1}^{H} \iota_{r, h}^{m}\left(x_{h}^{m}, a_{h}^{m}\right)+S_{r, H, 2}^{M}
\end{align*}
where $\left\{S_{r, h, k}^{m}\right\}_{(m, h, k) \in[M] \times[H] \times[2]}$ is a martingale scaling as $\widetilde{\mathcal{O}}\left( H^\frac{3}{2} M^\frac{1}{2}\right)$ via the Azuma-Hoeffding inequality.

From the recent work on the policy evaluation with UCB bonus \cite{jin2020provably,zhou2020nonstationary,touati2020efficient}, it can be shown that for every $(m,h) \in [M] \times [H]$ and $(x,a)\in \mathcal{S} \times \mathcal{A}$, with high probability, the cumulative model prediction error is bounded as
\begin{align*}
&\sum_{m=1}^M\sum_{h=1}^H \EE_{{\pi}^{\star,m}, \mathbb{P}^m} \left[ \iota_{r, h}^{m}(x_h,a_h) +\mu^m \iota_{g, h}^{m}(x_h,a_h)\right]  \\  &-\sum_{m=1}^{M} \sum_{h=1}^{H} \iota_{r, h}^{m}\left(x_{h}^{m}, a_{h}^{m}\right) \leq \widetilde{\mathcal{O}}\left( d^{\frac{9}{8}} H^{\frac{5}{2}} M^{\frac{3}{4}} B_\Delta^{\frac{1}{4}}\right).
\end{align*}
% \begin{align}\label{eq: model prediction error main paper}
% \nonumber &-2\left(\Gamma_{h}^{m}+\Gamma_{\diamond, h}^{m}\right)(x, a)-B_{\mathbb{P},\mathcal{E}} H^2 d_1^{\frac{3}{2}} W^\frac{1}{2} -B_{\diamond,\mathcal{E}} d_2^{\frac{1}{2}} W^{\frac{1}{2}} \\
% &\leq \iota_{\diamond, h}^{m}(x, a) \leq B_{\mathbb{P},\mathcal{E}} H^2 d_1^{\frac{3}{2}} W^\frac{1}{2} +B_{\diamond,\mathcal{E}} d_2^{\frac{1}{2}} W^{\frac{1}{2}},
% \end{align}
% where $B_{\mathbb{P},\mathcal{E}} \coloneqq \sum_{m=\ell^m}^{\ell^{m+1}-1}\sum_{h=1}^H \norm{\theta_h^m-\theta_h^{m-1}}_2$ and $B_{\diamond,\mathcal{E}} \coloneqq \sum_{m=\ell^m}^{\ell^{m+1}-1}\sum_{h=1}^H \norm{\theta_{\diamond, h}^m-\theta_{\diamond, h}^{m-1}}_2,  \label{eq: variation budget P}$ are the local variation budgets from the episodes $\ell^m$ to $\ell^{m+1}-1$. Note that we do not need to have the local variation budget information to derive our results. Thus, by choosing the appropriate window size $W$, we can bound the last term by ???

Finally, by combining the two terms (R.\rom{1}) and (R.\rom{2}) with \eqref{eq: decomposed d regret main paper}, we obtain the desired dynamic regret bound.


\subsection{Constraint violation analysis}
To analyze the constraint violation in \eqref{eq: Violation} under the non-stationarity condition, we also introduce a useful decomposition similar to \eqref{eq: decomposed d regret main paper} but weighted by the dual variable $\mu$. 

\begin{align} \label{eq: 16 1}
\nonumber & \sum_{m=1}^M \mu \left(b_m- V_{g,1}^{\pi^m,m} \right) \\
= &{\sum_{m=1}^M \mu \left(b_m-V_{g,1}^{m}(x_1) \right)} -\mu\text{MPE} + \mu S_{g, H, 2}^{M},
\end{align}
where $\text{MPE}$ is the term related to the model prediction error $\iota_{\diamond,h}^m$, and $S_{g, H, 2}^{M}$ is a martingale scaling as $\widetilde{\mathcal{O}}\left( H^\frac{5}{2} M^\frac{1}{2}\right)$ via the Azuma-Hoeffding inequality.
Using the similar procedure in the analysis of dynamic regret and noticing that $\left|\sum_{m=1}^M\left(V_{r, 1}^{\pi^{*,m},m}\left(x_{1}\right)- V_{r, 1}^{m}\left(x_{1}\right) \right)\right|\leq MH$, one can obtain
\begin{align} \label{eq: 17 1}
 &\sum_{m=1}^{M} \mu^{m}\left(b_m-V_{g, 1}^{m}\left(x_{1}\right)\right)\leq  \text{MPE} +S_{r, H, 2}^{M}\\
\nonumber & \hspace{1.5cm} + \widetilde{\mathcal{O}} \left(HM+H^3 M^{\frac{2}{3}} (\sqrt{d}B_\Delta+B_\star)^{\frac{1}{3}} \right),
% &{\sum_{m=1}^M\mu \left(V_{g,1}^{m}(x_1) -V_{g,1}^{\pi^m,m}(x_1)\right)}= \mu\text{MPE}_2 + \mu S_{g, H, 2}^{M},
\end{align}


To reduce the constraint violation under the non-stationarity condition, we fully utilize the dual regularization and the convexity of the Lagrangian with respect to the dual variable. In particular, with the dual regularization, we can  replace the iteration dependent $\mu^m$ with a fixed $\mu\geq 0$ as follows:
\begin{align} \label{eq: 18 1}
\hspace{-0.2cm} \sum_{m=1}^M (\mu-\mu^m) \left(b_m-V_{g,1}^{m} \right)-\sqrt{M}|\mu|^2    \leq \widetilde{\mathcal{O}}\left(H^2M^{\frac{1}{2}}\right).
\end{align}
By combining the equations \eqref{eq: 16 1}-\eqref{eq: 18 1} and adopting the dynamic regret analysis to control the model prediction errors, we obtain
\begin{align*}
& \mu \sum_{m=1}^M \left[ \left(b_m-V_{g, 1}^{\pi^m,m}\left(x_{1}\right)\right) - \widetilde{O} \left( d^{\frac{9}{8}}H^{\frac{7}{2}} M^{\frac{3}{4}} B_\Delta^{\frac{1}{4}} \right)\right] \\
&-\sqrt{M}|\mu|^2 \leq   \widetilde{\mathcal{O}}\left(d^{\frac{9}{8}}H^3 M (\sqrt{d}B_\Delta+B_\ast)^{\frac{1}{3}} \right).
\end{align*}
Since the above inequality holds for any $\mu\geq 0$, by maximizing the both sides of the above inequality over $\mu\geq 0$, i.e., choosing 
$\mu=\frac{\left(\sum_{m=1}^{M}\left(b_m-V_{g, 1}^{\pi^{m},m}\left(x_{1}\right) - \widetilde{O} \left( d^{\frac{9}{8}}H^{\frac{7}{2}} M^{\frac{3}{4}} B_\Delta^{\frac{1}{4}} \right)\right)\right)_+}{2\sqrt{M}}$,
we obtain the desired constraint violation bound.

% \subsection{Two time-scale periodic restart}
% To achieve our dynamic regret and constraint violation bound, we use a two time-scale periodic restart mechanisms: periodically restart the policy improvement with a 
% and periodically restart the optimistic policy evaluation with a 
% $L=$


==> files/checklist.tex <==
\section*{Checklist}
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} 
    % {\textit{As we stated in Section \ref{sec:intro}, this work only focuses on the optimization perspective of convex CMDP problems and does not study the sample complexity of the algorithm. Instead, we propose some alternative approaches to estimate the gradient of the Lagrangian function in Section \ref{subsec:gradient evaluation}.}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{} \textit{This is a theoretical study and to the best of our understanding it should not have any societal impacts.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNA{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
